Sanity Checks for Lottery Tickets: Does Your Winning Ticket Really Win the Jackpot?

There have been long-standing controversies and inconsistencies over the experiment setup and criteria for identifying the "winning ticket" in literature. To reconcile such, we revisit the definition of lottery ticket hypothesis, with comprehensive and more rigorous conditions. Under our new definition, we show concrete evidence to clarify whether the winning ticket exists across the major DNN architectures and/or applications. Through extensive experiments, we perform quantitative analysis on the correlations between winning tickets and various experimental factors, and empirically study the patterns of our observations. We find that the key training hyperparameters, such as learning rate and training epochs, as well as the architecture characteristics such as capacities and residual connections, are all highly correlated with whether and when the winning tickets can be identified. Based on our analysis, we summarize a guideline for parameter settings in regards of specific architecture characteristics, which we hope to catalyze the research progress on the topic of lottery ticket hypothesis. Our codes are publicly available at: https://github.com/boone891214/sanity-check-LTH.

==> fig_tex/main_mbv1_cf10.tex <==
\begin{figure*}[!h]
	\centering
	\begin{minipage}[b]{1.0\textwidth}
	\subfigure{
		\includegraphics[width=0.3\textwidth]{figs/main_results/mobilenetv1_cf10_0.832.pdf}
		\label{fig:mbv1_cf10_832}
	}
% 	\hfill
	\subfigure{
		\includegraphics[width=0.3\textwidth]{figs/main_results/mobilenetv1_cf10_0.914.pdf}
		\label{fig:mbv1_cf10_914}
	}
% 	\hfill
	\subfigure{
		\includegraphics[width=0.3\textwidth]{figs/main_results/mobilenetv1_cf10_0.945.pdf}
		\label{fig:mbv1_cf10_945}
	}
	\end{minipage}
	\caption{\red{explain why Jackpot, why secondary exist.}}
% 	\label{appendixfig:res20_cf10}
\label{fig:mbv1_cf10}
\end{figure*}

==> fig_tex/main_mbv1_cf100.tex <==
\begin{figure*}[!h]
	\centering
	\begin{minipage}[b]{1.0\textwidth}
	\subfigure{
		\includegraphics[width=0.3\textwidth]{figs/main_results/mobilenetv1_cf100_0.832.pdf}
		\label{fig:mbv1_cf100_832}
	}
% 	\hfill
	\subfigure{
		\includegraphics[width=0.3\textwidth]{figs/main_results/mobilenetv1_cf100_0.914.pdf}
		\label{fig:mbv1_cf100_914}
	}
% 	\hfill
	\subfigure{
		\includegraphics[width=0.3\textwidth]{figs/main_results/mobilenetv1_cf100_0.945.pdf}
		\label{fig:mbv1_cf100_945}
	}
	\end{minipage}
	\caption{\red{explain why Jackpot, why secondary exist.}}
\label{fig:mbv1_cf100}
\end{figure*}

==> fig_tex/main_res18_cf10.tex <==
\begin{figure*}[!h]
	\centering
	\begin{minipage}[b]{1.0\textwidth}
	\subfigure{
		\includegraphics[width=0.3\textwidth]{figs/main_results/resnet18_cf10_0.832.pdf}
		\label{fig:res18_cf10_832}
	}
% 	\hfill
	\subfigure{
		\includegraphics[width=0.3\textwidth]{figs/main_results/resnet18_cf10_0.914.pdf}
		\label{fig:res18_cf10_914}
	}
% 	\hfill
	\subfigure{
		\includegraphics[width=0.3\textwidth]{figs/main_results/resnet18_cf10_0.945.pdf}
		\label{fig:res18_cf10_945}
	}
	\end{minipage}
	\caption{\red{explain why Jackpot, why secondary exist.}}
% 	\label{appendixfig:res20_cf10}
\label{fig:res18_cf10}
\end{figure*}

==> fig_tex/main_res18_cf100.tex <==
\begin{figure*}[!h]
	\centering
	\begin{minipage}[b]{1.0\textwidth}
	\subfigure{
		\includegraphics[width=0.3\textwidth]{figs/main_results/resnet20_cf100_0.832.pdf}
		\label{fig:res20_cf100_832}
	}
% 	\hfill
	\subfigure{
		\includegraphics[width=0.3\textwidth]{figs/main_results/resnet20_cf100_0.914.pdf}
		\label{fig:res20_cf100_914}
	}
% 	\hfill
	\subfigure{
		\includegraphics[width=0.3\textwidth]{figs/main_results/resnet20_cf100_0.945.pdf}
		\label{fig:res20_cf100_945}
	}
	\end{minipage}
	\caption{\red{caption here!!!}}
% 	\label{appendixfig:res20_cf10}
\label{fig:res20_cf100}
\end{figure*}

==> fig_tex/main_res20_cf10.tex <==
\begin{figure*}[!h]
	\centering
	\begin{minipage}[b]{1.0\textwidth}
	\subfigure{
		\includegraphics[width=0.3\textwidth]{figs/main_results/resnet20_cf10_0.832.pdf}
		\label{fig:res20_cf10_832}
	}
% 	\hfill
	\subfigure{
		\includegraphics[width=0.3\textwidth]{figs/main_results/resnet20_cf10_0.914.pdf}
		\label{fig:res20_cf10_914}
	}
% 	\hfill
	\subfigure{
		\includegraphics[width=0.3\textwidth]{figs/main_results/resnet20_cf10_0.945.pdf}
		\label{fig:res20_cf10_945}
	}
	\end{minipage}
	\caption{\red{caption here!!!}}
% 	\label{appendixfig:res20_cf10}
\label{fig:res20_cf10}
\end{figure*}

==> fig_tex/main_res20_cf100.tex <==
\begin{figure*}[!h]
	\centering
	\begin{minipage}[b]{1.0\textwidth}
	\subfigure{
		\includegraphics[width=0.3\textwidth]{figs/main_results/resnet20_cf100_0.832.pdf}
		\label{fig:res20_cf100_832}
	}
% 	\hfill
	\subfigure{
		\includegraphics[width=0.3\textwidth]{figs/main_results/resnet20_cf100_0.914.pdf}
		\label{fig:res20_cf100_914}
	}
% 	\hfill
	\subfigure{
		\includegraphics[width=0.3\textwidth]{figs/main_results/resnet20_cf100_0.945.pdf}
		\label{fig:res20_cf100_945}
	}
	\end{minipage}
	\caption{\red{caption here!!!}}
% 	\label{appendixfig:res20_cf10}
\label{fig:res20_cf100}
\end{figure*}

==> fig_tex/main_res32_cf10.tex <==
\begin{figure*}[!h]
	\centering
	\begin{minipage}[b]{1.0\textwidth}
	\subfigure{
		\includegraphics[width=0.3\textwidth]{figs/main_results/resnet32_cf10_0.832.pdf}
		\label{fig:res32_cf10_832}
	}
% 	\hfill
	\subfigure{
		\includegraphics[width=0.3\textwidth]{figs/main_results/resnet32_cf10_0.914.pdf}
		\label{fig:res32_cf10_914}
	}
% 	\hfill
	\subfigure{
		\includegraphics[width=0.3\textwidth]{figs/main_results/resnet32_cf10_0.945.pdf}
		\label{fig:res32_cf10_945}
	}
	\end{minipage}
	\caption{\red{explain why Jackpot, why secondary exist.}}
% 	\label{appendixfig:res20_cf10}
\label{fig:res32_cf10}
\end{figure*}

==> fig_tex/main_res32_cf100.tex <==
\begin{figure*}[!h]
	\centering
	\begin{minipage}[b]{1.0\textwidth}
	\subfigure{
		\includegraphics[width=0.3\textwidth]{figs/main_results/resnet32_cf100_0.832.pdf}
		\label{fig:res32_cf100_832}
	}
% 	\hfill
	\subfigure{
		\includegraphics[width=0.3\textwidth]{figs/main_results/resnet32_cf100_0.914.pdf}
		\label{fig:res32_cf100_914}
	}
% 	\hfill
	\subfigure{
		\includegraphics[width=0.3\textwidth]{figs/main_results/resnet32_cf100_0.945.pdf}
		\label{fig:res32_cf100_945}
	}
	\end{minipage}
	\caption{\red{explain why Jackpot, why secondary exist.}}
% 	\label{appendixfig:res20_cf10}
\label{fig:res32_cf100}
\end{figure*}

==> fig_tex/main_vgg16_cf10.tex <==
\begin{figure*}[!h]
	\centering
	\begin{minipage}[b]{1.0\textwidth}
	\subfigure{
		\includegraphics[width=0.3\textwidth]{figs/main_results/vgg16_cf10_0.832.pdf}
		\label{fig:vgg16_cf10_832}
	}
% 	\hfill
	\subfigure{
		\includegraphics[width=0.3\textwidth]{figs/main_results/vgg16_cf10_0.914.pdf}
		\label{fig:vgg16_cf10_914}
	}
% 	\hfill
	\subfigure{
		\includegraphics[width=0.3\textwidth]{figs/main_results/vgg16_cf10_0.945.pdf}
		\label{fig:vgg16_cf10_945}
	}
	\end{minipage}
	\caption{\red{caption here!!!}}
\label{fig:vgg16_cf10}
\end{figure*}

==> fig_tex/main_vgg16_cf100.tex <==
\begin{figure*}[!h]
	\centering
	\begin{minipage}[b]{1.0\textwidth}
	\subfigure{
		\includegraphics[width=0.3\textwidth]{figs/main_results/vgg16_cf100_0.832.pdf}
		\label{fig:vgg16_cf100_832}
	}
% 	\hfill
	\subfigure{
		\includegraphics[width=0.3\textwidth]{figs/main_results/vgg16_cf100_0.914.pdf}
		\label{fig:vgg16_cf100_914}
	}
% 	\hfill
	\subfigure{
		\includegraphics[width=0.3\textwidth]{figs/main_results/vgg16_cf100_0.945.pdf}
		\label{fig:vgg16_cf100_945}
	}
	\end{minipage}
	\caption{\red{caption here!!!}}
\label{fig:vgg16_cf100}
\end{figure*}

==> sections/6_checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Please see Section~\ref{res:winning_ticket} and Appendix~\ref{apdx:exp_setups} in Supplemental material.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We report the details of the error bar settings in Section~\ref{res:winning_ticket}. The main results in Figure~\ref{fig:all_result_main} also includes variation data.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Please check Section~\ref{res:winning_ticket}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Source code will be provided, and we also properly cite the creators. Please refer to Appendix~\ref{apdx:exp_setups}.}
  \item Did you mention the license of the assets?
    \answerNA{We cite the orginial dataset and models.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We will provide all of our source code to reproduce the results.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{The datasets we use in this paper is public, and we cite the data providers.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{We use public dataset.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

